Continual Face Forgery Detection via Historical Distribution Preserving

Face forgery techniques have advanced rapidly and pose serious security threats. Existing face forgery detection methods try to learn generalizable features, but they still fall short of practical application. Additionally, finetuning these methods on historical training data is resource-intensive in terms of time and storage. In this paper, we focus on a novel and challenging problem: Continual Face Forgery Detection (CFFD), which aims to efficiently learn from new forgery attacks without forgetting previous ones. Specifically, we propose a Historical Distribution Preserving (HDP) framework that reserves and preserves the distributions of historical faces. To achieve this, we use universal adversarial perturbation (UAP) to simulate historical forgery distribution, and knowledge distillation to maintain the distribution variation of real faces across different models. We also construct a new benchmark for CFFD with three evaluation protocols. Our extensive experiments on the benchmarks show that our method outperforms the state-of-the-art competitors.

==> table/alg1.tex <==

\begin{algorithm}[t]
    \label{algorithm}
    \caption{UAP Generation }\label{algorithm}
    \begin{algorithmic}[1]%显示行号
        \Require{Real training dataset $D_{real}^t = \{x_{i},y_i=0\}_{i=1}^N$, $y_{fake}=1$,well trained t-th domain model $f^t(.)$, desired $l_{\infty}$ norm of perturbation $\epsilon$, learning rate $\alpha$, successful threshold $\sigma$}
        
        \Ensure{ $p_t = 1e^{-5}, M = 0$}
        \Repeat
            \For{each data $x_i \in D_{real}^t$}
            
                \Repeat
                    \State Calculate cross-entropy loss $L_{ce}((x_{i}+p_t),y_{fake};f^t)$.
                    \State Update $p_t$ by
                    \textit{E.q.}\ref{equation:eq1} 
                    \State\textbf{if} $||p_t||_{\infty}>\epsilon$ \textbf{then} clamp $p_t$ with $(-\epsilon,\epsilon)$
                \Until {$Pred(f^t(x_{i}+p_t;\theta,\phi)) \neq y_{i}$}
            \EndFor
            \State Count the number of successfully changed prediction results:
            \State $M = \frac{1}{N}\sum_{i=1}^{N}1(Pred(f^t(x_{i}+p_t;\theta,\phi)) \neq y_{i})$
            
        \Until{$M > N*\sigma$}
        \State\textbf{Return $p_t$}
        
        
    \end{algorithmic}
    \label{alg:main}
\end{algorithm}

==> table/alg_final.tex <==
\begin{algorithm}[h!]
    \label{algorithm}
    \caption{Historical Distribution Preserving }\label{algorithm}
    \begin{algorithmic}[1]%显示行号
        \Require{Sequence of  training dataset $D = \{D_{real}, D_{fake}^t\}_{t=1}^T$, initial model $f^0$, UAP pool $P$, desired $l_{\infty}$ norm of perturbation $\epsilon$, successful threshold $\sigma$.}
        
        \Ensure{ $P\leftarrow$\{\}}
        
            \For{\{$D_{real}$,$D^t_{fake}$\} $\in$ $D$}
            \If{$t==1$} 
                \State Optimize model $f^t$ with $L_{ce}^t$ on $D^t$. \Comment{Optimize the initial model.}
            \Else
                \Repeat
                \State Sample $p^n$ ($1<n<T$) from $P$. 
                \State Generate pseudo forgery set $D^n_p = p^n + D_{real}$.
                \State Optimize model $f^t$ with E.q.7 on $D^t$ and $D^n_p$. \Comment{Optimize the model via HDP.}
                \Until {Final epoch}
            \EndIf
            
            \State Set $p^{t} = 1e^{-5}, M = 0$.
            \Repeat \Comment{Generate UAP}
            \For{each data $x_i \in D_{real}$} 
                \Repeat
                    \State Calculate cross-entropy loss $L_{ce}((x_{i}+p^t),y_{fake};f^{t})$.
                    \State Update $p^t$ by
                    \textit{E.q.3}.
                    \State\textbf{if} $||p^t||_{\infty}>\epsilon$ \textbf{then} clamp $p^t$ with $(-\epsilon,\epsilon)$.
                \Until {$Pred(f^t(x_{i}+p^t;\theta,\phi)) \neq y_{i}$.}
            \EndFor
            \State Count the number of successfully changed prediction results:
            \State $M = \frac{1}{N}\sum_{i=1}^{N}1(Pred(f^t(x_{i}+p^t;\theta,\phi)) \neq y_{i})$
            
        \Until{$M > N*\sigma$}
            \State $P \leftarrow p^{t}$
            \EndFor
                
        \State\textbf{Return model $f^{T}$}
        
    \end{algorithmic}
    \label{alg:main}
\end{algorithm}


==> table/benchmark.tex <==
% \begin{table*}[!t]
%     \renewcommand\arraystretch{1.1}
%     \centering
    
%     \vspace{1pt}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|cc|cc|cc|cc|cc}
%         \hline
%         \multirow{2}*{Name} & \multicolumn{2}{c|}{Task1}&\multicolumn{2}{c|}{Task2} & \multicolumn{2}{c|}{Task3} & \multicolumn{2}{c|}{Task4} &\multicolumn{2}{c}{Task5}\\
%         \cline{2-11}
%         & Fake& Real &Fake& Real& Fake& Real& Fake& Real& Fake& Real\\
%         \hline
%         % \cline{2-11}
%         Protocol 1&Deepfakes&Mix&Face2Face&Mix&FaceSwap&Mix&NeuralTextures&Mix&Celeb-DF&Mix\\
%         Protocol 2&NeuralTextures&Mix&Deepfakes&Mix&Celeb-DF&Mix&Face2Face&Mix&FaceSwap&Mix\\
%         Protocol 3&Deepfakes&FF++&Face2Face&FF++&FaceSwap&FF++&NeuralTextures&FF++&Celeb-DF&Celeb-DF\\
        
%         \hline
%     \end{tabular}
    
%     }
%     \caption{Overview of the LFFD Benchmark. The Mix represents the mixture of two real samples of FF++ and Celeb-DF.}
%     \label{table:intro}
%     % \vspace{-0.5pt}
    
% \end{table*}


% \begin{table*}[!t]
%     \renewcommand\arraystretch{1.1}
%     \centering
    
%     \vspace{1pt}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{c|cc|cc|}
%         \hline
%         \multirow{2}*{Name} & \multicolumn{2}{c|}{Real}&\multicolumn{2}{c|}{Fake} \\
%         &Dataset&Number&Dataset&Number\\
%         Protocol1&\multirow{5}*{Real of FFpp and Celeb-DF}&\multirow{5}*2000&Deepfakes&2000\\

%         &&&Face2Face&2000\\
%         &&&FaceSwap&2000\\
%         &&&NeuralTextures&2000\\
%         &&&Celeb-DF&2000\\

%         Protocol2&\multirow{4}*{Real of Celeb}&\multirow{4}*2000&FFpp&2000\\

%         &&&Celeb-DF&2000\\
%         &&&Wild Deepfake&2000\\
%         &&&DFDC&2000\\
%         \hline
%     \end{tabular}
    
%     }
%     \caption{Overview of the LFFD Benchmark. The Mix represents the mixture of two real samples of FF++ and Celeb-DF.}
%     \label{table:intro}
%     % \vspace{-0.5pt}
    
% \end{table*}
% \begin{table*}[!t]
%     \renewcommand\arraystretch{1.1}
%     \centering
    
%     \vspace{1pt}
%     \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%         \hline
%         \multirow{2}*{Name} & \multirow{2}*{Dataset}&\multicolumn{3}{c|}{Fake Images}&\multicolumn{3}{c}{Real Images} \\
%         \cmidrule{3-8}

%         &&train&val&test&train&val&test\\
%         \hline

        
%         \multirow{5}*{Protocol1}&Deepfakes&11520&7000&7000&\multirow{5}*{11520}&\multirow{5}*{7000}&\multirow{5}*{7000}\\
%         &Face2Face&11520&7000&7000&&&\\
%         &FaceSwap&11520&7000&7000&&&\\
%         &NeuralTextures&11520&7000&7000&&&\\
%         % &Celeb-DF&79485&5100&5100&&&\\

%         \hline
%         \multirow{5}*{Protocol2}&FFpp&46080&28000&14000&\multirow{4}*{127592}&\multirow{4}*{26908}&\multirow{4}*{37003}\\
%         &Celeb-DF&79485&5100&7700&&&\\
%         &WildDeepfake&67800&9675&10250&&&\\
%         &DFDC&30849&6549&17398&&&\\
        


%         % &&&Face2Face&2000\\
%         % &&&FaceSwap&2000\\
%         % &&&NeuralTextures&2000\\
%         % &&&Celeb-DF&2000\\

%         % Protocol2&\multirow{4}*{Real of Celeb}&\multirow{4}*2000&FFpp&2000\\

%         % &&&Celeb-DF&2000\\
%         % &&&Wild Deepfake&2000\\
%         % &&&DFDC&2000\\
%         \hline
%     \end{tabular}
    
%     }
%     \caption{The LFFD benchmark with two protocols. The real images represents the summation of the number of real samples of the corresponding dataset, which are mixed in advance.}
%     \label{table:intro}

    
% \end{table*}
\begin{table*}[!t]
    \renewcommand\arraystretch{1.1}
    \centering
    
    \vspace{1pt}
    \resizebox{0.8\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
        \hline
        \multirow{2}*{Name} & \multirow{2}*{Dataset}&\multicolumn{3}{c|}{Fake Images}&\multicolumn{3}{c}{Real Images} \\
        \cmidrule{3-8}

        &&train&val&test&train&val&test\\
        \hline
        \multirow{5}*{Protocol 1}&Deepfakes&11520&7000&7000&\multirow{5}*{11520}&\multirow{5}*{7000}&\multirow{5}*{7000}\\
        &Face2Face&11520&7000&7000&&&\\
        &FaceSwap&11520&7000&7000&&&\\
        &NeuralTextures&11520&7000&7000&&&\\
        % &Celeb-DF&79485&5100&5100&&&\\

        \hline
        \multirow{5}*{Protocol 2}&FFpp&46080&28000&28000&11520&7000&7000\\

        &Celeb-DF&26495&8500&8500&17800&4450&4450\\
        &Wild-Deepfake&40680&5805&6150&44745&6390&5940\\
        &DFDC&30849&6549&17398&30832&6588&17433\\

        \hline
        \multirow{10}*{Protocol 3}&Deepfakes&11520&7000&7000&11520&7000&7000\\

        &Celeb-DF1&13277&4250&4250&8900&2224&2224\\
        &NeuralTextures&11520&7000&7000&11520&7000&7000\\
        &Wild-Deepfake1&20340&2902&3075&22372&3195&2970\\
        &FaceSwap&11520&7000&7000&11520&7000&7000\\
        &DFDC1&15424&3274&8699&15416&3294&8716\\
        &Face2Face&11520&7000&7000&11520&7000&7000\\
        &Celeb-DF2&13277&4250&4250&8900&2224&2224\\
        &Wild-Deepfake2&20340&2902&3075&22372&3195&2970\\
        &DFDC2&15424&3274&8699&15416&3294&8716\\
        \hline
    \end{tabular}
    }
    \caption{Details of CFFD benchmark with three protocols.}
    \label{table:intro}
\end{table*}


==> table/mix_ablation.tex <==

\begin{figure}
\small
\begin{minipage}[t]{0.6\linewidth}
\centering
\begin{centering}
	\setlength{\tabcolsep}{1mm}{
		\vspace{-0.10in}
		\scalebox{1.1}{ %
			\begin{tabular}{c}
				\begin{tabular}{c|c|c|c|c|c|c}
        \hline
        
        \multirow{2}*{Base Training}&\multirow{2}*{FDP}& \multirow{2}*{RDP} &\multicolumn{2}{c|}{Protocol1}&\multicolumn{2}{c}{Protocol2}\\
        \cmidrule{4-7}

        &&& AVG &PRE& AVG &PRE\\
        \hline
        \checkmark&&&75.05&67.29&57.71&47.53\\
        \checkmark&\checkmark&&77.17&74.33&59.00&48.84\\
        \checkmark&&\checkmark&81.58&81.19&62.19&56.34\\
        \checkmark&\checkmark&\checkmark&\textbf{93.32}&\textbf{94.94}&\textbf{70.10}&\textbf{76.68}\\

        \hline
    \end{tabular}\tabularnewline
	\end{tabular}}}
% 	\vspace{0.05in}
	\captionof{table}{Ablation study on the influence of different components on protocol1 and protocol2 in terms of ACC. The FDP represents the Forgery distribution Preserving strategy and the RDP represents the Real Distribution Preserving strategy.}
		\label{Tab:ablation}
	\vspace{-0.10in}
	\par\end{centering}
\end{minipage}
\hspace{0.10in}	
\begin{minipage}[t]{0.38\linewidth} 
	\centering 
	\vspace{-0.1in}
	\includegraphics[width=0.8\linewidth]{NIPS/figures/uap2.pdf}
	\vspace{-0.1in}
	\caption{Visualization of the UAP for Deepfakes and NeuralTexture, respectively. More results are reported in supplementary material.
	\label{fig:uap}}
	\vspace{-0.10in}
\end{minipage}
\end{figure}

==> table/protocol1.tex <==
\begin{table*}[!t]
    \renewcommand\arraystretch{1.1}
    \centering
    
    \vspace{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc|cc}
        \hline
        \multirow{2}*{Method} &Buffer &\multicolumn{2}{c|}{Deepfakes}&\multicolumn{2}{c|}{Face2Face} & \multicolumn{2}{c|}{FaceSwap} & \multicolumn{2}{c|}{NeuralTextures} &\multicolumn{2}{c|}{Celeb-DF}&\multicolumn{2}{c|}{AVG}&\multicolumn{2}{c}{PRE}\\
        \cmidrule{3-16}
        &/Step & ACC& AUC &ACC& AUC& ACC& AUC& ACC& AUC& ACC& AUC& ACC& AUC& ACC& AUC\\
        \hline
        % \cline{2-11}
        SFT&0&57.36&56.50&57.35&45.08&57.35&37.26&57.35&52.25&\textbf{99.10}&\textbf{99.97}&65.70&58.01&64.00&72.03\\
        LwF&0&58.02&82.67&57.80&71.65&57.52&71.65&57.80&73.51&98.96&99.92&66.02&79.99&67.57&86.36\\
        MAS&0&62.05&92.23&57.38&63.55&57.13&57.73&57.48&60.88&98.78&99.94&66.56&74.86&73.66&81.89\\
        NCM&0&61.47&60.26&61.67&44.13&61.41&34.62&61.65&54.62&99.37&99.97&69.11&58.72&66.09&72.02\\
        % NCM*&0&57.97&45.89&62.40&64.80&65.31&64.04&62.87&58.69&98.90&99.17&69.49&66.51&66.09&72.02\\
        % NCM*&0&61.74&60.26&61.67&63.55&57.13&57.73&57.48&60.88&98.78&99.94&66.56&74.86&73.65&81.89\\

        % ICaLR-100&75.19&87.93&73.87&88.71&70.91&87.00&66.16&77.04&98.38&99.93&76.90&88.12&78.31&90.37\\

        iCaRL&500&59.53&89.50&57.83&70.53&57.64&79.00&57.63&66.15&99.30&99.97&66.38&81.03&73.04&88.25\\
        SCR&500&62.05&92.23&57.38&63.55&57.13&57.73&57.48&60.88&98.78&99.94&66.56&74.86&73.65&81.89\\
        FReTAL&500&60.37&92.55&57.86&73.18&57.18&61.25&60.18&84.64&98.24&99.83&66.76&82.29&72.40&89.01\\
        DER&500&85.24&93.17&72.29&79.49&65.90&71.69&70.51&78.14&90.21&99.71&76.83&84.44&73.69&79.71\\
        DER++&500&87.38&94.10&73.15&82.32&68.62&76.25&68.11&76.77&93.13&99.77&78.07&85.84&77.88&85.40\\
        Co2L&500&80.27&74.29&73.51&86.63&70.13&86.53&65.31&76.56&97.37&99.69&77.42&84.74&75.43&85.80\\
        \hline
        Ours&1&\textbf{90.64}&\textbf{96.37}&\textbf{76.67}&\textbf{88.25}&\textbf{88.08}&\textbf{96.46}&\textbf{72.42}&\textbf{84.14}&97.34&99.76&\textbf{85.03}&\textbf{92.99}&\textbf{89.74}&\textbf{95.62}\\
        \hline
        Joint&-&97.25&99.65&96.88&98.74&97.38&99.15&92.91&97.18&98.83&99.88&96.65&98.92&-&-\\
        \hline
    \end{tabular}
    
    }
    \caption{Quantitative results on protocol1 in terms of ACC and AUC. We evaluate the last model on all the previous test sets. The buffer represents the memory bank budget for each step.}
    \label{table:protocol1}
    % \vspace{-0.5pt}
    
\end{table*}


==> table/protocol2.tex <==
\begin{table*}[!t]
    \renewcommand\arraystretch{1.1}
    \centering
    
    \vspace{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc|cc}
        \hline
        \multirow{2}*{Method} &Buffer &\multicolumn{2}{c|}{NeuralTextures}&\multicolumn{2}{c|}{Deepfakes} & \multicolumn{2}{c|}{Celeb-DF} & \multicolumn{2}{c|}{Face2Face} &\multicolumn{2}{c|}{FaceSwap}&\multicolumn{2}{c|}{AVG}&\multicolumn{2}{c}{PRE}\\
        \cmidrule{3-16}
        &/Task & ACC& AUC &ACC& AUC& ACC& AUC& ACC& AUC& ACC& AUC& ACC& AUC& ACC& AUC\\
        \hline
        % \cline{2-11}
        SFT&0&57.95&60.75&64.99&84.84&65.23&44.57&67.19&89.99&\textbf{98.98}&99.53&70.86&75.93&63.16&71.66\\
        LwF&0&58.01&76.56&66.50&90.45&65.26&88.84&68.08&86.63&98.93&99.27&71.34&88.35&64.08&87.34\\
        MAS&0&76.59&88.72&75.30&89.17&63.51&30.55&78.13&88.57&95.96&99.11&77.89&79.22&73.13&76.77\\
        NCM*&0&58.04&63.29&66.43&87.75&65.27&49.70&69.53&92.28&98.00&99.17&71.45&78.43&71.45&78.43\\
        % NCM*&0&57.97&45.89&62.40&64.80&65.31&64.04&62.87&58.69&98.90&99.17&69.49&66.51&66.09&72.02\\
        % NCM*&0&57.97&45.89&62.40&64.80&65.31&64.04&62.87&58.69&98.90&99.17&69.49&66.51&61.91&60.54\\

        % ICaLR-100&75.19&87.93&73.87&88.71&70.91&87.00&66.16&77.04&98.38&99.93&76.90&88.12&78.31&90.37\\

        iCaRL&500&58.13&68.96&65.59&90.89&65.00&38.72&69.86&92.81&98.69&
        \textbf{99.75}&71.45&78.22&66.88&76.99\\
        SCR*&500&58.48&80.70&\textbf{86.54}&\textbf{98.22}&65.36&23.05&75.49&95.85&99.07&97.99&76.98&79.16&69.19&79.65\\
        FReTAL&500&61.24&87.17&72.36&91.45&66.43&92.17&79.48&94.80&98.05&99.00&75.51&92.91&70.64&91.93\\
        DER&500&57.90&55.45&69.98&78.64&65.25&30.66&84.43&87.16&98.81&99.42&75.24&70.26&65.16&67.19\\
        DER++&500&57.46&61.78&72.07&80.78&56.45&38.14&88.30&95.57&90.55&99.37&72.96&75.12&66.44&65.84\\
        Co2L&500&58.57&63.20&78.41&90.12&65.00&41.17&77.44&87.76&97.60&99.17&75.40&76.28&67.71&71.93\\
        \hline
        Ours&1&\textbf{78.87}&\textbf{91.26}&74.46&95.10&\textbf{73.37}&\textbf{93.63}&\textbf{96.13}&\textbf{98.33}&97.80&99.18&\textbf{84.12}&\textbf{95.50}&\textbf{80.43}&\textbf{95.25}\\
        \hline
        Joint&-&97.25&99.65&96.88&98.74&97.38&99.15&92.91&97.18&98.83&99.88&96.65&98.92&-&-\\
        \hline
    \end{tabular}
    }
    \caption{Overview of the LFFD Benchmark. The Mix represents the mixture of two real samples of FF++ and Celeb-DF.}
    \label{table:order2}
    % \vspace{-0.5pt}
    
\end{table*}


==> table/protocol3.tex <==
\begin{table*}[!t]
    \renewcommand\arraystretch{1.1}
    \centering
    
    \vspace{1pt}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|cc|cc|cc|cc|cc|cc}
        \hline
        \multirow{2}*{Method} &Buffer &\multicolumn{2}{c|}{FFpp}&\multicolumn{2}{c|}{Celeb-DF} & \multicolumn{2}{c|}{WildDeepfake} & \multicolumn{2}{c|}{DFDC} &\multicolumn{2}{c|}{AVG}&\multicolumn{2}{c}{PRE}\\
        \cmidrule{3-14}
        &/Step & ACC& AUC & ACC& AUC& ACC& AUC& ACC& AUC& ACC& AUC& ACC& AUC\\
        \hline
        % \cline{2-11}
        SFT&0&56.59&82.06&35.22&72.70&50.85&56.67&88.21&95.67&57.71&76.77&47.53&70.88\\
        LwF&0&61.30&85.13&35.49&83.49&53.36&81.88&88.38&\textbf{95.76}&59.63&86.56&51.54&84.68\\
        MAS&0&70.10&68.33&35.46&26.78&54.08&54.74&85.00&93.51&61.16&60.84&55.98&65.68\\
        NCM&0&59.07&74.60&36.78&62.15&51.28&59.67&87.70&93.32&58.70&72.43&48.81&66.03\\

        iCaRL&500&60.95&83.29&40.72&71.06&52.23&64.95&88.15&95.65&60.51&78.73&50.13&76.72\\
        SCR&500&62.72&70.66&35.70&39.88&53.14&61.99&88.19&59.85&59.93&58.09&50.60&70.72\\
        FReTAL&500&64.88&92.37&38.29&90.17&57.57&84.17&87.91&95.77&62.16&90.62&51.25&89.25\\
        DER&500&58.68&76.35&34.88&37.55&50.55&53.28&87.79&95.65&57.97&65.70&48.46&66.44\\
        DER++&500&59.78&80.28&40.07&68.75&51.76&54.52&87.43&95.90&59.76&74.86&52.75&74.63\\
        % Co2L&500&&&&&&&&&&&&\\
        \hline
        Ours&1&\textbf{83.78}&\textbf{96.45}&\textbf{50.78}&\textbf{96.88}&\textbf{57.95}&\textbf{85.42}&\textbf{88.95}&95.33&\textbf{70.36}&\textbf{93.52}&\textbf{76.68}&\textbf{95.77}\\
        \hline
        Joint&-&96.05&99.67&98.53&99.89&83.39&90.40&87.56&96.60&91.88&96.64&-&-\\
        \hline
    \end{tabular}
    
    }
    \caption{Quantitative results on protocol2. We evaluate the last model on the test sets of all tasks in terms of ACC and AUC. The training order is FFpp->Celeb-DF->WildDeepfake->DFDC.}
    \label{table:protocol2}
    % \vspace{-0.5pt}
    
\end{table*}

